Fine-tuning Diffusion Policies with Backpropagation Through Diffusion Timesteps

Diffusion policies, widely adopted in decision-making scenarios such as robotics, gaming and autonomous driving, are capable of learning diverse skills from demonstration data due to their high representation power. However, the sub-optimal and limited coverage of demonstration data could lead to diffusion policies that generate sub-optimal trajectories and even catastrophic failures. While reinforcement learning (RL)-based fine-tuning has emerged as a promising solution to address these limitations, existing approaches struggle to effectively adapt Proximal Policy Optimization (PPO) to diffusion models. This challenge stems from the computational intractability of action likelihood estimation during the denoising process, which leads to complicated optimization objectives. In our experiments starting from randomly initialized policies, we find that online tuning of Diffusion Policies demonstrates much lower sample efficiency compared to directly applying PPO on MLP policies (MLP+PPO). To address these challenges, we introduce NCDPO, a novel framework that reformulates Diffusion Policy as a noise-conditioned deterministic policy. By treating each denoising step as a differentiable transformation conditioned on pre-sampled noise, NCDPO enables tractable likelihood evaluation and gradient backpropagation through all diffusion timesteps. Our experiments demonstrate that NCDPO achieves sample efficiency comparable to MLP+PPO when training from scratch, outperforming existing methods in both sample efficiency and final performance across diverse benchmarks, including continuous robot control and multi-agent game scenarios. Furthermore, our experimental results show that our method is robust to the number denoising timesteps in the Diffusion Policy.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/07_checklist.tex <==
\section{Reproducibility Statement}
All necessary source code for {\METHOD} and modified BDPO and DAC baselines are submitted in the supplementary materials. For other baselines, please refer to DPPO github page.

% \newpage
% \section*{NeurIPS Paper Checklist}



% \begin{enumerate}

% \item {\bf Claims}
%     \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Our main contribution, a novel framework for Diffusion Policy fine-tuning is properly described in the abstract and introduction.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
%         \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
%         \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
%         \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
%     \end{itemize}

% \item {\bf Limitations}
%     \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
%     \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Limitations are mentioned in the conclusion.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
%         \item The authors are encouraged to create a separate "Limitations" section in their paper.
%         \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
%         \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
%         \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
%         \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
%         \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
%         \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
%     \end{itemize}

% \item {\bf Theory assumptions and proofs}
%     \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: We do not have theory included.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include theoretical results. 
%         \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
%         \item All assumptions should be clearly stated or referenced in the statement of any theorems.
%         \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
%         \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
%         \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
%     \end{itemize}

%     \item {\bf Experimental result reproducibility}
%     \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: We have clearly described the algorithm in the main text and listed all necessary details in the appendix.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include experiments.
%         \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
%         \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
%         \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
%         \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
%         \begin{enumerate}
%             \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
%             \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
%             \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
%             \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
%         \end{enumerate}
%     \end{itemize}


% \item {\bf Open access to data and code}
%     \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: We have included the details and will release code and datasets soon.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that paper does not include experiments requiring code.
%         \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
%         \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
%         \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
%         \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
%         \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
%         \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
%         \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
%     \end{itemize}


% \item {\bf Experimental setting/details}
%     \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: We have listed details in appendix.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include experiments.
%         \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
%         \item The full details can be provided either with the code, in appendix, or as supplemental material.
%     \end{itemize}

% \item {\bf Experiment statistical significance}
%     \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: We averaged results over at least 3 different seeds and reports mean and standard deviation. Meanwhile, the performance advantage is significant enough.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include experiments.
%         \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
%         \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
%         \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
%         \item The assumptions made should be given (e.g., Normally distributed errors).
%         \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
%         \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
%         \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
%         \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
%     \end{itemize}

% \item {\bf Experiments compute resources}
%     \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: We have provided compute resources in appendix.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include experiments.
%         \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
%         \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
%         \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
%     \end{itemize}
    
% \item {\bf Code of ethics}
%     \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification:  Yes, we followed the NeurIPS Code of Ethics.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
%         \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
%         \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
%     \end{itemize}


% \item {\bf Broader impacts}
%     \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
%     \item[] Answer: \answerNA{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Our paper focus on designing a novel training framework, and no societal impact.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that there is no societal impact of the work performed.
%         \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
%         \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
%         \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
%         \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
%         \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
%     \end{itemize}
    
% \item {\bf Safeguards}
%     \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Our paper has no such risks.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper poses no such risks.
%         \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
%         \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
%         \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
%     \end{itemize}

% \item {\bf Licenses for existing assets}
%     \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Datasets are cited in main text, code is cited in Appendix~\ref{appendix:implementation}
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not use existing assets.
%         \item The authors should cite the original paper that produced the code package or dataset.
%         \item The authors should state which version of the asset is used and, if possible, include a URL.
%         \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
%         \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
%         \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
%         \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
%         \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
%     \end{itemize}

% \item {\bf New assets}
%     \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: We have included our code and dataset in supplementary materials.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not release new assets.
%         \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
%         \item The paper should discuss whether and how consent was obtained from people whose asset is used.
%         \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
%     \end{itemize}

% \item {\bf Crowdsourcing and research with human subjects}
%     \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
%         \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
%         \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
%     \end{itemize}

% \item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
%     \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
%         \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
%         \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
%         \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
%     \end{itemize}

% \item {\bf Declaration of LLM usage}
%     \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
%     %this research? 
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: LLM is only used for paper language refinement and code auto-completion.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
%         \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
%     \end{itemize}

% \end{enumerate}

==> sec/back_5_exp.tex <==
\section{Experiments}

In this section, we present a comprehensive evaluation of  {\METHOD} across a variety of environments. These environments range from continuous control tasks to multi-agent centralized control with discrete action space. Our evaluation set provides a robust framework for assessing the versatility and effectiveness of {\METHOD}. 
% The experiments illustrate the capacity of {\METHOD} to fine-tune a diffusion policy, showcasing its adaptability and efficiency in handling a wide range of environments. {\METHOD} consistently demonstrates strong and stable performance across multiple testbeds, including those with continuous and discrete action spaces, as well as varying configurations of action chunk sizes and diffusion denoising steps.

\paragraph{Environments: OpenAI Gym.} Our first set of experiments involved testing {\METHOD} on a series of well-established locomotion benchmarks from OpenAI Gym \citep{brockman2016openai}, namely: \texttt{Hopper-v2}, \texttt{Walker2D-v2}, and \texttt{HalfCheetah-v2}. The pre-trained diffusion policies used in these experiments are trained from the D4RL "medium" dataset \citep{fu2020d4rl}, which contains a diverse range of pre-recorded trajectories. For the fine-tuning process, we employed \textbf{dense} reward. 
% \gjx{don't use words like "were" or "tested"}

\paragraph{Environments: Robomimic.} We further evaluate the performance of METHOD on robotic manipulation tasks within Robomimic benchmarks~\citep{robomimic2021}.  The specific scenarios we considered include \texttt{Lift}, \texttt{Can}, \texttt{Square}, and \texttt{Transport}, which vary in difficulty. To maintain consistency in action and ensure a high success rate for the pre-trained models, \yny{we apply \textbf{action chunking}, a common practice in robot manipulation tasks.} Specifically, we set the action chunk size to 4 for the \texttt{Lift}, \texttt{Can}, and \texttt{Square} tasks, and to 8 for the more challenging \texttt{Transport} task, \yny{aligning with the settings in DPPO paper~\citep{ren2024diffusion}.} Notably, these tasks are fine-tuned using \textbf{sparse} rewards, which provide feedback only in the form of success or failure signals, representing a more challenging learning scenario for RL algorithms.
% \gjx{It seems no need to introduce chunk size here...  it is merely a hyperparamter that does not relate to the algorithm} \yny{Action chunk is very important for robomimic's performance, also we need to remind the readers that our tests aligns with those of DPPO.}
% \sout{These benchmarks are designed to test the performance of reinforcement learning agents in more complex, high-dimensional manipulation tasks.}

\textbf{Environments: Google Research Football.} To evaluate the effectiveness of {\METHOD} in large action space, we selecte three representative scenarios from Google Research Football \citep{kurach2020google}: \texttt{3 vs 1 with Keeper}, \texttt{Counterattack Hard}, and \texttt{Corner}. \yny{These environments all involve multi-agent control. We adopt a centralized control approach, where actions for all agents are generated simultaneously using a single diffusion policy. The base diffusion policies are pre-trained to output one-hot vectors corresponding to ground-truth actions. To construct the pre-training dataset, we aggregate trajectories from multiple MLP-based policies with varying success rates.} 
% \gjx{make this part simple. you only need to present two things: 1. we use a multi-agent centralized control setting that features a large action space. 2. we construct the demonstration datasets by collecting trajectories from policies trained with MAPPO.}



% \paragraph{Baselines.} To evaluate the effectiveness of our proposed method, we conduct a comparative analysis against existing approaches. Specifically, we compared {{\METHOD}} \yny{with Diffusion Policy Optimization (DPPO) \citep{ren2024diffusion}, \textbf{DRWR}, \textbf{DAWR} \citep{ren2024diffusion}, \textbf{DIPO} \citep{yang2023policy}, \textbf{IDQL} \citep{hansen2023idql} and \textbf{DQL} \citep{wang2022diffusion}, in both the \textbf{Robomimic} and \textbf{OpenAI Gym locomotion tasks} environments}, and with Multi-Agent Proximal Policy Optimization (MAPPO) \citep{yu2022surprising}, adopting MLP as base model, in the \textbf{Google Research Football} environment. To ensure a fair comparison, we also employed cross-entropy loss to pre-train MLP. \gjx{@yny: where are the other baselines? you should talk about ALL baselines}
\paragraph{Baselines.} To evaluate the effectiveness of our proposed method, we conduct a comprehensive comparative analysis against existing approaches. \yny{Specifically, we compare \textbf{{\METHOD}} with several baselines, including \textbf{DPPO} \citep{ren2024diffusion}; \textbf{DRWR} and \textbf{DAWR}, both proposed in the DPPO paper and based on reward-weighted regression and advantage-weighted regression respectively; \textbf{DIPO} \citep{yang2023policy}, which employs action gradients as the score function for denoising steps; and Q-learning-based methods such as \textbf{IDQL} \citep{hansen2023idql} and \textbf{DQL} \citep{wang2022diffusion}.}
% \gjx{@yny: where are the other baselines? you should talk about ALL baselines}


\subsection{Main Results}

\yny{{\METHOD} demonstrates superior performance and sample efficiency across a diverse set of environments. In the following sections, we provide a detailed analysis of the experimental results for each setting.}

% \sout{We also included other various baselines for comparison: \textbf{DRWR}, \textbf{DAWR}, which are based on reward-weighted regression and advantage-weighted regression proposed in DPPO paper \citep{ren2024diffusion}, \textbf{DIPO} \citep{yang2023policy}, which utilizes the action gradient as score function for denoising steps, as well as Q-learning based methods including \textbf{IDQL} \citep{hansen2023idql} and \textbf{DQL} \citep{wang2022diffusion}. For a fair comparison, we set the action chunk size to match the size in DPPO paper.\yny{maybe move this part to "baseline" above?}}
% Furthermore, in the 



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/gym.png}
%     \caption{Performance comparison on OpenAI Gym locomotion tasks. Results are averaged over three seeds.}
%     \label{fig:gym}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/robomimic.png}
%     \caption{Performance comparison on Robomimic tasks. Results are averaged over three seeds.}
%     \label{fig:robomimic}
% \end{figure}


\textbf{Continuous Robot Control.}
% Our method demonstrates superior performance in the OpenAI Gym locomotion environments, outperforming the DPPO~\citep{ren2024diffusion} baseline in both sample efficiency and final performance. In the Robomimic environment, {\METHOD} achieves comparable results to DPPO, indicating its effectiveness across diverse settings. 
From the experimental results shown in Figures~\ref{fig:gym} and~\ref{fig:robomimic}, we observe that {\METHOD} consistently achieves the strongest performance and robustness across all tasks. While our main baseline, DPPO, performs comparably to {\METHOD} in the Robomimic benchmark \footnote{Note that we tested performance using the latest version of DPPO (v0.8), which is about 2.5x sample efficient as reported in the original paper.}, it lags behind in the OpenAI Gym locomotion environments. Other baselines generally underperform relative to DPPO. Notably, IDQL demonstrates strong performance on the first three Robomimic tasks but fails in the final one. In contrast, DQL suffers from instability across all scenarios.






\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/gym.png}
    \caption{Performance comparison on OpenAI Gym locomotion tasks. Results are averaged over three seeds. {\METHOD} (ours) achieves the strongest performance.}
    \label{fig:gym}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/robomimic.png}
    \caption{Performance comparison on Robomimic tasks. Results are averaged over three seeds. {\METHOD} (ours) achieves the strongest performance.}
    \label{fig:robomimic}
\end{figure}


\begin{table}[H]
\label{sample-table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Scenario     &{\METHOD} (Ours) & DPPO & AWR & IDQL & DQL & RWR & DIPO \\
\midrule
Hopper-Medium      & \textbf{3297.3} (47.8)  & 2566.6 (51.1) & 1168.9 (30.5) & 2970.2 (5.2)  & 3200.7 (30.1)  & 2633.6 (94.0)  & 2463.1 (127.6) \\
Hopper-Medium-Replay & \textbf{3345.64} (71.88) & 2988.97 (86.90) & 2142.30 (183.82) & 3076.91 (29.82) & 3159.72 (94.85) & 2718.27 (79.86) & 2834.07 (25.00) \\
Hopper-Medium-Expert & \textbf{3528.74} (51.89) & 2672.64 (135.15) & 1062.47 (13.15) & 3440.50 (10.79) & 3153.66 (733.36) & 2964.11 (121.35) & 3326.99 (32.73) \\
Walker2d-Medium    & \textbf{4248.8} (137.6) & 3632.1 (55.9) & 3353.9 (296.9) & 3972.8 (17.3) & 3405.2 (1322.7) & 3238.3 (116.8) & 3581.6 (70.3) \\
Walker2d-Medium-Replay & \textbf{4544.59} (162.98) & 3770.52 (154.50) & 2719.04 (83.84) & 4373.89 (91.66) & 3846.26 (1357.97) & 2483.04 (215.70) & 3180.80 (396.27) \\
Walker2d-Medium-Expert & \textbf{5060.92} (82.87) & 4935.57 (73.28) & 4458.68 (195.26) & 4863.91 (95.34) & 2416.68 (1708.34) & 3831.65 (243.76) & 4979.96 (50.22) \\
HalfCheetah & \textbf{7058.8} (635.1) & 4758.3 (41.8) & 3788.7 (166.5) & 4584.4 (45.3) & 4459.1 (309.5) & 2773.1 (310.0) & 4272.4 (33.2) \\

HalfCheetah-Expert & \textbf{8079.30} (392.21) & 4663.23 (92.62) & 3723.21 (131.37) & 4499.39 (57.61) & 4171.97 (465.25) & 2218.39 (168.36) & 4126.96 (12.14) \\

HalfCheetah-Replay & \textbf{7000.14} (113.88) & 4181.57 (24.59) & 3501.08 (40.34) & 4295.81 (53.02) & 4223.07 (177.28) & 1775.98 (101.28) & 3362.48 (49.47) \\

\hline

Lift & \textbf{1.00} (0.00) & 0.997 (0.0029) & 0.933 (0.0176) & 0.992 (0.0104) & 0.998 (0.003) & 0.975 (0.005) & 0.973 (0.008) \\
Can & \textbf{0.993} (0.012) & 0.990 (0.010) & 0.338 (0.032) & 0.945 (0.031) & 0.003 (0.006) & 0.907 (0.008) & 0.528 (0.051) \\
Square & \textbf{87.33} (4.51) & 87.0 (2.29) & 40.33 (8.50) & 80.0 (5.0) & 0.0 (0.0) & 74.83 (2.57) & 25.33 (4.54) \\
Transport & \textbf{96.67} (2.31) & 91.33 (2.93) & 11.17 (3.51) & 0.50 (0.87) & 0.0 (0.0) & 0.0 (0.0) & 0.17 (0.29) \\
\bottomrule
\end{tabular}%
}
\caption{Mean and standard deviation of performance across continuous robot control scenarios. Each result is evaluated on three different seeds. {\METHOD} (ours) exhibits the strongest performance.}
\label{table:performance}

% \caption{Average evaluation reward and standard deviation (over three seeds) on OpenAI Gym Mujoco. The base diffusion policies are all pretrained on D4RL medium datasets.}
\end{table}



% \begin{table}[H]
% \label{sample-table}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% Scenario     &{\METHOD} (Ours) & DPPO & AWR & IDQL & DQL & RWR & DIPO \\
% \midrule
% Hopper-Medium      & \textbf{3297} (48)  & 2567 (51) & 1169 (31) & 2970 (5)  & 3201 (30)  & 2634 (94)  & 2463 (128) \\
% Hopper-Medium-Replay & \textbf{3346} (72) & 2989 (87) & 2142 (184) & 3077 (30) & 3160 (95) & 2718 (80) & 2834 (25) \\
% Hopper-Medium-Expert & \textbf{3529} (52) & 2673 (135) & 1062 (13) & 3441 (11) & 3154 (733) & 2964 (121) & 3327 (33) \\
% Walker2d-Medium    & \textbf{4249} (138) & 3632 (56) & 3354 (297) & 3973 (17) & 3405 (1323) & 3238 (117) & 3582 (70) \\
% Walker2d-Medium-Replay & \textbf{4545} (163) & 3771 (155) & 2719 (84) & 4374 (92) & 3846 (1358) & 2483 (216) & 3180 (396) \\
% Walker2d-Medium-Expert & \textbf{5061} (83) & 4936 (73) & 4459 (195) & 4864 (95) & 2417 (1708) & 3832 (244) & 4980 (50) \\
% HalfCheetah & \textbf{7059} (635) & 4758 (42) & 3789 (167) & 4584 (45) & 4459 (310) & 2773 (310) & 4272 (33) \\
% HalfCheetah-Expert & \textbf{8079} (392) & 4663 (93) & 3723 (131) & 4499 (58) & 4172 (465) & 2218 (168) & 4127 (12) \\
% HalfCheetah-Replay & \textbf{7000} (114) & 4182 (25) & 3501 (40) & 4296 (53) & 4223 (177) & 1776 (101) & 3362 (49) \\
% \hline

% Lift & \textbf{100.0} (0.0) & 99.7 (0.2) & 93.3 (1.7) & 99.2 (0.1) & 99.8 (0.3) & 97.5 (0.5) & 97.3 (0.8) \\
% Can & \textbf{99.3} (1.2) & 99.0 (1.0) & 33.8 (3.2) & 94.5 (3.1) & 0.3 (0.6) & 90.7 (0.8) & 52.8 (5.1) \\
% Square & \textbf{87.3} (4.5) & 87.0 (2.3) & 40.3 (8.5) & 80.0 (5.0) & 0.0 (0.0) & 74.8 (2.5) & 25.3 (4.5) \\
% Transport & \textbf{96.7} (2.31) & 91.3 (2.9) & 11.2 (3.5) & 0.5 (0.8) & 0.0 (0.0) & 0.0 (0.0) & 0.2 (0.3) \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Mean and standard deviation of performance across continuous robot control scenarios. Each result is evaluated on three different seeds. {\METHOD} (ours) exhibits the strongest performance.}
% \label{table:performance}

% % \caption{Average evaluation reward and standard deviation (over three seeds) on OpenAI Gym Mujoco. The base diffusion policies are all pretrained on D4RL medium datasets.}
% \end{table}



\begin{table}[H]
\label{sample-table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Scenario     &{\METHOD} (Ours) & DPPO & AWR & IDQL & DQL & RWR & DIPO \\
\midrule
Hopper-Medium          & \textbf{101.95} (1.48) & 79.33 (1.58) & 36.14 (0.94) & 91.84 (0.16) & 98.96 (0.93) & 81.42 (2.91) & 76.17 (3.95) \\
Hopper-Medium-Replay   & \textbf{103.44} (2.22) & 92.42 (2.69) & 66.24 (5.68) & 95.12 (0.92) & 97.69 (2.93) & 84.01 (2.47) & 87.65 (0.77) \\
Hopper-Medium-Expert   & \textbf{109.10} (1.60) & 82.66 (4.18) & 32.86 (0.41) & 106.38 (0.33) & 97.50 (22.68) & 91.65 (3.75) & 102.87 (1.01) \\
Walker2d-Medium        & \textbf{92.53} (3.00)  & 79.09 (1.22) & 73.04 (6.47) & 86.52 (0.38) & 74.17 (28.80) & 70.51 (2.54) & 77.99 (1.53) \\
Walker2d-Medium-Replay & \textbf{98.96} (3.55)  & 82.12 (3.36) & 59.20 (1.83) & 95.24 (1.99) & 83.75 (29.57) & 54.06 (4.70) & 69.26 (8.63) \\
Walker2d-Medium-Expert & \textbf{110.21} (1.81) & 107.47 (1.60) & 97.08 (4.25) & 105.91 (2.08) & 52.61 (37.22) & 83.44 (5.31) & 108.45 (1.09) \\
HalfCheetah            & \textbf{58.17} (5.23)  & 39.22 (0.34) & 31.22 (1.37) & 37.78 (0.37) & 36.74 (2.55) & 22.85 (2.55) & 35.21 (0.27) \\
HalfCheetah-Expert     & \textbf{66.57} (3.23)  & 38.43 (0.76) & 30.67 (1.08) & 37.08 (0.47) & 34.38 (3.83) & 18.28 (1.39) & 34.01 (0.10) \\
HalfCheetah-Replay     & \textbf{57.69} (0.94)  & 34.47 (0.20) & 28.85 (0.33) & 35.39 (0.44) & 34.81 (1.46) & 14.63 (0.83) & 27.71 (0.41) \\

\hline

Lift & \textbf{100.0} (0.0) & 99.7 (0.2) & 93.3 (1.7) & 99.2 (0.1) & 99.8 (0.3) & 97.5 (0.5) & 97.3 (0.8) \\
Can & \textbf{99.3} (1.2) & 99.0 (1.0) & 33.8 (3.2) & 94.5 (3.1) & 0.3 (0.6) & 90.7 (0.8) & 52.8 (5.1) \\
Square & \textbf{87.3} (4.5) & 87.0 (2.3) & 40.3 (8.5) & 80.0 (5.0) & 0.0 (0.0) & 74.8 (2.5) & 25.3 (4.5) \\
Transport & \textbf{96.7} (2.31) & 91.3 (2.9) & 11.2 (3.5) & 0.5 (0.8) & 0.0 (0.0) & 0.0 (0.0) & 0.2 (0.3) \\
\bottomrule
\end{tabular}%
}
\caption{Mean and standard deviation of performance across continuous robot control scenarios. Each result is evaluated on three different seeds. {\METHOD} (ours) exhibits the strongest performance.}
\label{table:performance}

% \caption{Average evaluation reward and standard deviation (over three seeds) on OpenAI Gym Mujoco. The base diffusion policies are all pretrained on D4RL medium datasets.}
\end{table}

% \begin{table}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% Scenario & DiffPPO & DPPO & AWR & IDQL & DQL & RWR & DIPO \\
% \midrule
% Lift & 99.33 (0.58) & 99.83 (0.29) & 88.50 (4.09) & \textbf{100.0} (0.0) & 99.83 (0.29) & 97.50 (2.00) & 98.50 (0.87) \\
% Can & \textbf{100.0} (0.0) & 99.0 (1.0) & 33.83 (3.21) & 94.50 (3.12) & 0.33 (0.58) & 90.67 (0.76) & 52.83 (5.11) \\
% Square & \textbf{87.33} (4.51) & 87.0 (2.29) & 40.33 (8.50) & 80.0 (5.0) & 0.0 (0.0) & 74.83 (2.57) & 25.33 (4.54) \\
% Transport & \textbf{96.67} (2.31) & 91.33 (2.93) & 11.17 (3.51) & 0.50 (0.87) & 0.0 (0.0) & 0.0 (0.0) & 0.17 (0.29) \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Mean and standard deviation of performance across different scenarios.}
% \label{table:performance}
% \end{table}




\textbf{Discrete Multi-agent Control.}
In Google Research Football environment, {\METHOD} significantly outperforms the MLP baseline across all three evaluated scenarios. Here we adopt a \textbf{centralized multi-agent control strategy} to fully leverage the representational power of diffusion models. Instead of independently generating each agent’s action, a single diffusion model simultaneously produces the action probability logits for all agents—resulting in an expanded joint action space. As shown in Fig.~\ref{fig:football}, {\METHOD} is capable of handling environments with such large action spaces.

% These results collectively highlight the robust performance of {\METHOD} in both continuous and discrete action spaces. \gjx{@yny: this paragraph could be shortened into sth like "{\METHOD} demonstrates superior performance and sample efficiency across a wide range of environments. Here we analyze the main results one by one.". discuss the results of {\METHOD} in the following different sections is fine}

% In Google Research Football, 

Since we are unaware of any existing baselines that fine-tune diffusion policies with discrete action spaces using online interaction, we compare only with a basic MLP+PPO setup, initialized via conducting behavior cloning with Cross-Entropy loss. \yny{Training curves show that while MLP+PPO struggles to capture complex behaviors from the demonstration dataset, DP+{\METHOD} effectively learns from more diverse and intricate pre-training data.}

% In Google Research Football, we adopt multi-agent centralized control to better exploit the power of diffusion model. Instead of independently generating each agents' actions, we calculate all agents' action probability logits using a single diffusion model, resulting in expanded action space. Results in ~\ref{fig:football} demonstrates {\METHOD} is powerful enough to handle environments with large action space. Since we could not find other baseline that fine-tunes a diffusion policy with discrete action space using online interaction, we only compares with basic MLP+PPO, initialized by conducting behavior cloning with Cross-Entropy loss. \yny{Training curves indicate that while MLP+PPO fails to capture complex behaviors in demonstration dataset, DP+DiffPPO can effectively handle complicated pre-training data.}

% Dataset for pre-training base policies are composed of trajectories with diverse action modes. As there is no available dataset for Google Research Football, we built our own dataset by training and early-stopping multiple training with different seeds using MAPPO\citep{yu2022surprising}. These agents have different winning rates and are observed to adopt diverse tactics.

The dataset used for pre-training base policies consists of trajectories exhibiting diverse action modes. Since no public dataset is available for Google Research Football, we construct our own by training multiple MAPPO agents~\citep{yu2022surprising} with different random seeds and early-stopping them at various stages. These agents demonstrate varying winning rates and are observed to employ diverse tactical behaviors, thereby enriching the dataset with a wide range of strategies.



% In Robomimic, datasets are collected by 6 different human operators. D4RL datasets are generated by training an agent using Soft Actor-Critic \citep{haarnoja2018soft}, early-stopping it and then use it to generate interaction trajectories. 

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/football.png}
    \caption{Performance comparison in Google Research Football. Results are averaged over five seeds. \yny{{\METHOD} (ours) exhibits strong performance and stability.}}
    \label{fig:football}
\end{figure}


\begin{table}[H]
  \label{football}
  \centering
  \begin{tabular}{lll}
    \toprule
    % \multicolumn{2}{c}{Part}                   \\
    % \cmidrule(r){1-3}
    Scenario     & {\METHOD} (Ours)     & MAPPO \\
    \midrule
    3v1 &  \textbf{87.4}(2.7) &  {75}(12.3)  \\
    CA\_hard  & \textbf{87.0}(2.5) &  {80.0}(2.0) \\
    Corner     &   \textbf{74.9}(3.07)  &  {74.2}(5.1) \\
    \bottomrule
  \end{tabular}
  \caption{Average evaluation success rate and standard deviation (over three seeds) on Google Research Football scenarios. The base diffusion policy and MLP policy are pre-trained on the same dataset. MLP policy is trained using Cross-Entropy loss. }
\end{table}


% \subsection{Diverse Demonstration Data}



% \gjx{@yny: analyze the experiment results}


\subsection{Ablation Study}

We further conduct an ablation study to investigate the impact of varying the number of denoising steps in the diffusion model. The experimental results shown in Fig.~\ref{fig:ablation-denoise_step} indicate that {\METHOD} demonstrates strong robustness to the choice of denoising steps.
% , maintaining stable performance across a wide range of settings.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/gym-denoise.png}
    \caption{Ablation Study on Denoising Steps in OpenAI Gym locomotion tasks.}
    \label{fig:ablation-denoise_step}
\end{figure}


We hypothesize that the robustness of {\METHOD} arises from the way gradients are propagated through time during the diffusion process. This temporal gradient flow leads to more accurate gradient estimates without introducing latent actions.

% We also conduct ablation studies on action chunk size and diffusion noise scheduler in \ref{sec_ablation}.
% Such characteristics enable our policy to learn from more direct signals provided by the environment, while also benefiting from the well-established advantages of PPO in reinforcement learning. Additionally, the expressive power of the diffusion model in the pre-training phase contributes significantly to the learning a strong base policy.


==> sec/back_5_exp_2.tex <==
\section{Experiments}

In this section, we provide a comprehensive empirical evaluation of {\METHOD} across a range of challenging environments. We begin by detailing the experimental setup in Sec.\ref{sec:setup}, followed by results on continuous robot control tasks in Sec.\ref{sec:continuous} and discrete multi-agent coordination tasks in Sec.\ref{sec:discrete}. Finally, we conduct ablation studies in Sec.\ref{sec:ablation} to assess the robustness and of {\METHOD}.

% Our testbeds consist of  tasks and multi-agent coordination tasks with high-dimensional discrete action space.  For the continuous control benchmarks, we compare {\METHOD} against recent diffusion policy RL baselines. For the discrete multi-agent settings, where no established diffusion-based online RL baseline exists, we benchmark {\METHOD} against a standard MLP+PPO approach.


% Our evaluation set provides a comprehensive assessment for the versatility and effectiveness of {\METHOD}. 
% The experiments illustrate the capacity of {\METHOD} to fine-tune a diffusion policy, showcasing its adaptability and efficiency in handling a wide range of environments. {\METHOD} consistently demonstrates strong and stable performance across multiple testbeds, including those with continuous and discrete action spaces, as well as varying configurations of action chunk sizes and diffusion denoising steps.


\subsection{Environments and Baselines\label{sec:setup}}

\paragraph{Environments: OpenAI Gym locomotion.} Our first set of experiments involved testing {\METHOD} on a series of well-established locomotion benchmarks from OpenAI Gym \citep{brockman2016openai}, namely: \texttt{Hopper-v2}, \texttt{Walker2D-v2}, and \texttt{HalfCheetah-v2}. The pre-trained diffusion policies used in these experiments are trained from the D4RL "medium" dataset \citep{fu2020d4rl}, which contains a diverse range of pre-recorded trajectories. For the fine-tuning process, we employed \textbf{dense} reward. 
% \gjx{don't use words like "were" or "tested"}

% \paragraph{Environments: Robomimic.} We further evaluate the performance of METHOD on robotic manipulation tasks within Robomimic benchmarks~\citep{robomimic2021}.  The specific scenarios we considered include \texttt{Lift}, \texttt{Can}, \texttt{Square}, and \texttt{Transport}, which vary in difficulty. To maintain consistency in action and ensure a high success rate for the pre-trained models, \yny{we apply \textbf{action chunking}, a common practice in robot manipulation tasks.} Specifically, we set the action chunk size to 4 for the \texttt{Lift}, \texttt{Can}, and \texttt{Square} tasks, and to 8 for the more challenging \texttt{Transport} task, \yny{aligning with the settings in DPPO paper~\citep{ren2024diffusion}.} Notably, these tasks are fine-tuned using \textbf{sparse} rewards, which provide feedback only in the form of success or failure signals, representing a more challenging learning scenario for RL algorithms.
\paragraph{Environments: Robomimic.} We further evaluate the performance of METHOD on robotic manipulation tasks within Robomimic benchmarks~\citep{robomimic2021}.  The specific scenarios we considered include \texttt{Lift}, \texttt{Can}, \texttt{Square}, and \texttt{Transport}, varying in difficulty. \yny{To ensure temporal consistency in actions, we employ action chunking with size 4 for \texttt{Lift}, \texttt{Can}, and \texttt{Square}, and size 8 for \texttt{Transport}, following the setting in~\citep{ren2024diffusion}.} All tasks are fine-tuned using \textbf{sparse} rewards, which provide feedback only in the form of success or failure signals. 
% \yny{Datasets for pre-training are collected by 6 different human operators~\citep{robomimic2021}.}
% \gjx{It seems no need to introduce chunk size here...  it is merely a hyperparamter that does not relate to the algorithm} \yny{Action chunk is very important for robomimic's performance, also we need to remind the readers that our tests aligns with those of DPPO.}
% \sout{These benchmarks are designed to test the performance of reinforcement learning agents in more complex, high-dimensional manipulation tasks.}

\textbf{Environments: Google Research Football.} 
\yny{To evaluate {\METHOD}'s scalability in large discrete action spaces, we test on three Google Research Football scenarios requiring multi-agent coordination: \texttt{3 vs 1 with Keeper}, \texttt{Counterattack Hard}, and \texttt{Corner}.}
% To evaluate the effectiveness of {\METHOD} in large action space, we select three representative scenarios from Google Research Football \citep{kurach2020google}: \texttt{3 vs 1 with Keeper}, \texttt{Counterattack Hard}, and \texttt{Corner}.
\yny{Here we adopt a centralized control approach, where actions for all agents are generated simultaneously using a single diffusion policy. The base diffusion policies are pre-trained to output one-hot vectors corresponding to ground-truth actions. To construct the pre-training dataset, we aggregate trajectories from multiple MLP-based policies with varying success rates.} 
% \gjx{make this part simple. you only need to present two things: 1. we use a multi-agent centralized control setting that features a large action space. 2. we construct the demonstration datasets by collecting trajectories from policies trained with MAPPO.}



% \paragraph{Baselines.} To evaluate the effectiveness of our proposed method, we conduct a comparative analysis against existing approaches. Specifically, we compared {{\METHOD}} \yny{with Diffusion Policy Optimization (DPPO) \citep{ren2024diffusion}, \textbf{DRWR}, \textbf{DAWR} \citep{ren2024diffusion}, \textbf{DIPO} \citep{yang2023policy}, \textbf{IDQL} \citep{hansen2023idql} and \textbf{DQL} \citep{wang2022diffusion}, in both the \textbf{Robomimic} and \textbf{OpenAI Gym locomotion tasks} environments}, and with Multi-Agent Proximal Policy Optimization (MAPPO) \citep{yu2022surprising}, adopting MLP as base model, in the \textbf{Google Research Football} environment. To ensure a fair comparison, we also employed cross-entropy loss to pre-train MLP. \gjx{@yny: where are the other baselines? you should talk about ALL baselines}
\paragraph{Baselines.} To evaluate the effectiveness of our proposed method, we conduct a comprehensive comparative analysis against existing approaches. \yny{Specifically, in  OpenAI Gym locomotion and Robomimic, we compare \textbf{{\METHOD}} with \textbf{DPPO} \citep{ren2024diffusion}; \textbf{DRWR} and \textbf{DAWR}, both proposed in the DPPO paper and based on reward-weighted regression and advantage-weighted regression respectively; \textbf{DIPO} \citep{yang2023policy}, which employs action gradients as the score function for denoising steps; and Q-learning-based methods such as \textbf{IDQL} \citep{hansen2023idql} and \textbf{DQL} \citep{wang2022diffusion}.} In Google Research Football, we compare with Multi-Agent Proximal Policy Optimization (MAPPO) \citep{yu2022surprising}, adopting MLP as base model. MLP policy is initialized via pre-training with Cross-Entropy loss.
% \gjx{@yny: where are the other baselines? you should talk about ALL baselines}


% \subsection{Main Results\label{sec:main}}

% \yny{Experimental results shows that {\METHOD} demonstrates remarkable performance and sample efficiency across a diverse set of environments. In the following sections, we provide a detailed analysis of the experimental results for each setting.}

% \sout{We also included other various baselines for comparison: \textbf{DRWR}, \textbf{DAWR}, which are based on reward-weighted regression and advantage-weighted regression proposed in DPPO paper \citep{ren2024diffusion}, \textbf{DIPO} \citep{yang2023policy}, which utilizes the action gradient as score function for denoising steps, as well as Q-learning based methods including \textbf{IDQL} \citep{hansen2023idql} and \textbf{DQL} \citep{wang2022diffusion}. For a fair comparison, we set the action chunk size to match the size in DPPO paper.\yny{maybe move this part to "baseline" above?}}
% Furthermore, in the 



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/gym.png}
%     \caption{Performance comparison on OpenAI Gym locomotion tasks. Results are averaged over three seeds.}
%     \label{fig:gym}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/robomimic.png}
%     \caption{Performance comparison on Robomimic tasks. Results are averaged over three seeds.}
%     \label{fig:robomimic}
% \end{figure}


% \textbf{Continuous Robot Control.}
\subsection{Evaluation on Continuous Robot Control Tasks.\label{sec:continuous}}
% Our method demonstrates superior performance in the OpenAI Gym locomotion environments, outperforming the DPPO~\citep{ren2024diffusion} baseline in both sample efficiency and final performance. In the Robomimic environment, {\METHOD} achieves comparable results to DPPO, indicating its effectiveness across diverse settings. 
\yny{We first evaluate {\METHOD} on continuous control tasks across two benchmarks: OpenAI Gym locomotion and Robomimic.}
From the experimental results shown in Figures~\ref{fig:gym} and~\ref{fig:robomimic}, we observe that {\METHOD} consistently achieves the strongest performance and robustness across all tasks. While our main baseline, DPPO, performs comparably to {\METHOD} in the Robomimic benchmark \footnote{Note that we tested performance using the latest version of DPPO (v0.8), which is about 2.5x sample efficient as reported in the original paper.}, it lags behind in the OpenAI Gym locomotion environments. Other baselines generally underperform relative to DPPO. Notably, IDQL demonstrates strong performance on the first three Robomimic tasks but fails in the final one. In contrast, DQL suffers from instability across all scenarios.






\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/gym.png}
    \caption{Performance comparison on OpenAI Gym locomotion tasks. Results are averaged over three seeds. {\METHOD} (ours) achieves the strongest performance.}
    \label{fig:gym}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/robomimic.png}
    \caption{Performance comparison on Robomimic tasks. Results are averaged over three seeds. {\METHOD} (ours) achieves the strongest performance.}
    \label{fig:robomimic}
\end{figure}

% \caption{Average evaluation reward and standard deviation (over three seeds) on OpenAI Gym Mujoco. The base diffusion policies are all pretrained on D4RL medium datasets.}
\begin{table}[H]
\label{sample-table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Scenario     &{\METHOD} (Ours) & DPPO & AWR & IDQL & DQL & RWR & DIPO \\
\midrule
Hopper-Medium         & \textbf{101.9} (1.5)  & 79.4 (1.6)   & 36.1 (0.9)   & 91.8 (0.2)   & 99.0 (0.9)   & 81.4 (2.9)   & 76.2 (3.9) \\
Hopper-Medium-Replay  & \textbf{103.4} (2.2)  & 92.4 (2.7)   & 66.2 (5.7)   & 95.1 (0.9)   & 97.7 (2.9)   & 84.0 (2.5)   & 87.6 (0.8) \\
Hopper-Medium-Expert  & \textbf{109.1} (1.6)  & 82.6 (4.2)   & 32.9 (0.4)   & 106.4 (0.3)  & 97.5 (22.7)  & 91.6 (3.8)   & 102.9 (1.0) \\

Walker2d-Medium       & \textbf{92.5} (3.0)   & 79.1 (1.2)   & 73.0 (6.5)   & 86.5 (0.4)   & 74.2 (28.8)  & 70.5 (2.5)   & 78.0 (1.5) \\
Walker2d-Medium-Replay& \textbf{99.0} (3.5)   & 82.1 (3.4)   & 59.2 (1.8)   & 95.2 (2.0)   & 83.8 (29.6)  & 54.1 (4.7)   & 69.3 (8.6) \\
Walker2d-Medium-Expert& \textbf{110.2} (1.8)  & 107.5 (1.6)  & 97.1 (4.3)   & 105.9 (2.1)  & 52.6 (37.2)  & 83.4 (5.3)   & 108.4 (1.1) \\

HalfCheetah-Medium     & \textbf{58.2} (5.2)   & 39.2 (0.3)   & 31.2 (1.4)   & 37.8 (0.4)   & 36.7 (2.6)   & 22.9 (2.6)   & 35.2 (0.3) \\
HalfCheetah-Medium-Expert & \textbf{66.6} (3.2) & 38.4 (0.8)   & 30.7 (1.1)   & 37.1 (0.5)   & 34.4 (3.8)   & 18.3 (1.4)   & 34.0 (0.1) \\
HalfCheetah-Medium-Replay & \textbf{57.7} (0.9) & 34.5 (0.2)   & 28.9 (0.3)   & 35.4 (0.4)   & 34.8 (1.5)   & 14.6 (0.8)   & 27.7 (0.4) \\

\hline

Lift & \textbf{100.0} (0.0) & 99.7 (0.2) & 93.3 (1.7) & 99.2 (0.1) & 99.8 (0.3) & 97.5 (0.5) & 97.3 (0.8) \\
Can & \textbf{99.3} (1.2) & 99.0 (1.0) & 33.8 (3.2) & 94.5 (3.1) & 0.3 (0.6) & 90.7 (0.8) & 52.8 (5.1) \\
Square & \textbf{87.3} (4.5) & 87.0 (2.3) & 40.3 (8.5) & 80.0 (5.0) & 0.0 (0.0) & 74.8 (2.5) & 25.3 (4.5) \\
Transport & \textbf{96.7} (2.31) & 91.3 (2.9) & 11.2 (3.5) & 0.5 (0.8) & 0.0 (0.0) & 0.0 (0.0) & 0.2 (0.3) \\
\bottomrule
\end{tabular}%
}
\caption{Mean and standard deviation of performance over continuous robot control scenarios. Each result is evaluated on three different seeds. {\METHOD} (ours) exhibits the strongest performance. Performance on  OpenAI Gym locomotion tasks are normalized according to scores of SAC reported in D4RL ~\citep{fu2020d4rl}. Original scores are listed in Table~\ref{table:performance_original}.}
\label{table:performance}

% \caption{Average evaluation reward and standard deviation (over three seeds) on OpenAI Gym Mujoco. The base diffusion policies are all pretrained on D4RL medium datasets.}
\end{table}

% \textbf{\yny{Discrete Multi-agent Coordination.}}
\subsection{Evaluation on Discrete Multi-agent Coordination Tasks.\label{sec:discrete}}
\yny{Following our evaluation on continuous control tasks, we next examine {\METHOD} on Google Research Football, a benchmark for cooperative multi-agent control. To fully exploit the representational capacity of diffusion models, we adopt a centralized multi-agent control strategy where actions for all agents are generated simultaneously. This strategy results in a high-dimensional joint action space (i.e., $\text{num\_agents} \times \text{actions}$), which poses significant challenges for conventional methods.}

\yny{Since no existing baseline fine-tunes diffusion policies with discrete action spaces using online interaction, we compare {\METHOD} only with a standard MLP+PPO setup. This baseline is initialized through behavior cloning using a Cross-Entropy loss function.}
The dataset for pre-training the base policies consists of trajectories with diverse action modes. As no public dataset exists for Google Research Football, a custom dataset was constructed by training multiple MAPPO agents~\citep{yu2022surprising} with different random seeds and early-stopping them at various stages. These agents exhibit varying winning rates and employ diverse tactical behaviors, thereby enriching the dataset with a broad range of strategies.

\yny{As Fig.~\ref{fig:football} demonstrates, {\METHOD} outperforms the MLP baseline across all three evaluated scenarios. This outcome not only highlights the superiority of diffusion policy in handling complex and diverse demonstration data over simple MLP policy, but also confirms the effectiveness of the DP+{\METHOD} during the fine-tuning phase.}


% \yny{Following our evaluation on continuous control tasks, we then evaluate {\METHOD} on Google Research Football, a multi-agent cooperation benchmark. To harness the full representational capacity of diffusion models, we adopt a centralized multi-agent control strategy, wherein actions for all agents are generated simultaneously. This approach naturally leads to a high-dimensional joint action space ($\text{num\_agents} \times \text{actions}$), posing significant challenges for conventional methods. Nevertheless, as shown in Fig.~\ref{fig:football}, {\METHOD} excels at tackling environments with such high-dimensional action spaces.}

% \yny{Since we are unaware of any existing baselines that fine-tune diffusion policies with discrete action spaces using online interaction, we compare only with a basic MLP+PPO setup, initialized via conducting behavior cloning with Cross-Entropy loss.}
% The dataset used for pre-training base policies consists of trajectories exhibiting diverse action modes. Since no public dataset is available for Google Research Football, we construct our own by training multiple MAPPO agents~\citep{yu2022surprising} with different random seeds and early-stopping them at various stages. These agents demonstrate varying winning rates and are observed to employ diverse tactical behaviors, thereby enriching the dataset with a wide range of strategies.

% As Fig.~\ref{fig:football} shows, {\METHOD} outperforms the MLP baseline across all three evaluated scenarios. \yny{ This not only demonstrates the superiority of diffusion policy over simple MLP policy when pretraining from datasets with diverse modes, but also corroborates the effectiveness of DP+{\METHOD}, beating MLP+PPO in the fine-tuning phase.}



\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/football.png}
    \caption{Performance comparison in Google Research Football. Results are averaged over at least three seeds. \yny{{\METHOD} (ours) exhibits strong performance and stability.}}
    \label{fig:football}
\end{figure}


\begin{table}[H]
  \label{football}
  \centering
  \begin{tabular}{lll}
    \toprule
    % \multicolumn{2}{c}{Part}                   \\
    % \cmidrule(r){1-3}
    Scenario     & {\METHOD} (Ours)     & MAPPO \\
    \midrule
    3 vs 1 with Keeper &  \textbf{87.4}(2.7) &  {75.1}(12.3)  \\
    Counterattack Hard  & \textbf{87.0}(2.5) &  {80.0}(2.0) \\
    Corner     &   \textbf{78.3}(4.5)  &  {74.9}(3.0) \\
    \bottomrule
  \end{tabular}
  \caption{Average evaluation success rate and standard deviation (over three seeds) on Google Research Football scenarios. The base diffusion policy and MLP policy are pre-trained on the same dataset. MLP policy is trained using Cross-Entropy loss. 
  }
\end{table}


% \subsection{Diverse Demonstration Data}



% \gjx{@yny: analyze the experiment results}


\subsection{Ablation Study\label{sec:ablation}}

We further conduct an ablation study to investigate the impact of varying the number of denoising steps in the diffusion model. The experimental results shown in Fig.~\ref{fig:ablation-denoise_step} indicate that {\METHOD} demonstrates strong robustness to the choice of denoising steps.
% , maintaining stable performance across a wide range of settings.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/gym-denoise.png}
    \caption{Ablation Study on Denoising Steps in OpenAI Gym locomotion tasks.}
    \label{fig:ablation-denoise_step}
\end{figure}


We hypothesize that the robustness of {\METHOD} arises from the way gradients are propagated through time during the diffusion process. This gradient flow leads to more accurate gradient estimates.
% without introducing latent actions.

% We also conduct ablation studies on action chunk size and diffusion noise scheduler in \ref{sec_ablation}.
% Such characteristics enable our policy to learn from more direct signals provided by the environment, while also benefiting from the well-established advantages of PPO in reinforcement learning. Additionally, the expressive power of the diffusion model in the pre-training phase contributes significantly to the learning a strong base policy.


==> sec/denoising.tex <==
\begin{figure}[htbp]
    \centering
\resizebox{1.0\textwidth}{!}{
\begin{tikzpicture}[scale=1.0, transform shape, % Other options remain the same
    font=\large\sffamily,
    every node/.style={align=center},
    node distance=0.7cm and 1.4cm,
    >={Stealth[round]},
    thick
]


% Define row positioning
\def\forwardrow{0}
\def\noiserow{2.5}
\def\srow{-2} % Row for S node

% Define color-specific batch stacking styles with black borders and proper stacking order
\tikzset{
    blue batch stack/.style={
            preaction={
                  fill=blue!15,
                  draw=black,
                  line width=0.5pt,
                  opacity=0.4,
                  transform canvas={xshift=12pt, yshift=-12pt}
            },
            preaction={
                  fill=blue!20,
                  draw=black,
                  line width=0.5pt,
                  opacity=0.5,
                  transform canvas={xshift=8pt, yshift=-8pt}
            },
            preaction={
                  fill=blue!25,
                  draw=black,
                  line width=0.5pt,
                  opacity=0.6,
                  transform canvas={xshift=4pt, yshift=-4pt}
            }
    },
    green batch stack/.style={
        preaction={
            fill=green!15,
            draw=black,
            line width=0.5pt,
            opacity=0.4,
            transform canvas={xshift=12pt, yshift=-12pt}
        },
        preaction={
            fill=green!20,
            draw=black,
            line width=0.5pt,
            opacity=0.5,
            transform canvas={xshift=8pt, yshift=-8pt}
        },
        preaction={
            fill=green!25,
            draw=black,
            line width=0.5pt,
            opacity=0.6,
            transform canvas={xshift=4pt, yshift=-4pt}
        }
    },
    yellow batch stack/.style={
        preaction={
            fill=yellow!15,
            draw=black,
            line width=0.5pt,
            opacity=0.4,
            transform canvas={xshift=12pt, yshift=-12pt}
        },
        preaction={
            fill=yellow!20,
            draw=black,
            line width=0.5pt,
            opacity=0.5,
            transform canvas={xshift=8pt, yshift=-8pt}
        },
        preaction={
            fill=yellow!25,
            draw=black,
            line width=0.5pt,
            opacity=0.6,
            transform canvas={xshift=4pt, yshift=-4pt}
        }
    }
}

% ----- FORWARD PATH NODES (NOW HORIZONTAL) -----
% a^t (initial noise)
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.7cm,
      minimum height=1cm,
      top color=blue!10,
      bottom color=blue!25,
      blue batch stack,
      at={(0,\forwardrow)}
] (at) {\(a^t\)};

% a^{t-1}
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.7cm,
      minimum height=1cm,
      top color=green!10,
      bottom color=green!25,
      green batch stack,
      right= of at
] (atm1) {\(a^{t-1}\)};

\node[right=3cm of atm1] (dots) {\(\ldots\)};

% a^2
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.7cm,
      minimum height=1cm,
      top color=green!10,
      bottom color=green!25,
      green batch stack,
      right= 3cm of dots
] (a2) {\(a^2\)};

% a^1
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.7cm,
      minimum height=1cm,
      top color=green!10,
      bottom color=green!25,
      green batch stack,
      right=of a2
] (a1) {\(a^1\)};

% a^0
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.7cm,
      minimum height=1cm,
      top color=green!10,
      bottom color=green!25,
      green batch stack,
      right=of a1
] (a0) {\(a^0\)};

% Place S directly below the dots node (which is already centered)
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.7cm,
      minimum height=1cm,
      top color=blue!10,
      bottom color=blue!25,
      blue batch stack,
      below=2.5cm of dots,
      label={[yshift=-0.5cm]below:{\textbf{Observation}}}
] (S) {\(S\)};

% Extract x-coordinates of state nodes
\path let \p1 = (at.center) in \pgfextra{\xdef\atx{\x1}};
\path let \p1 = (atm1.center) in \pgfextra{\xdef\atmonex{\x1}};
\path let \p1 = (a2.center) in \pgfextra{\xdef\atwox{\x1}};
\path let \p1 = (a1.center) in \pgfextra{\xdef\aonex{\x1}};

% Place noise nodes with exact x-coordinate alignment
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.2cm,
      minimum height=0.8cm,
      top color=yellow!10,
      bottom color=yellow!25,
      yellow batch stack
] (zt) at (\atx, \noiserow) {\(z^t\)};

\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.2cm,
      minimum height=0.8cm,
      top color=yellow!10,
      bottom color=yellow!25,
      yellow batch stack
] (ztm1) at (\atmonex, \noiserow) {\(z^{t-1}\)};

\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.2cm,
      minimum height=0.8cm,
      top color=yellow!10,
      bottom color=yellow!25,
      yellow batch stack
] (z2) at (\atwox, \noiserow) {\(z^2\)};

\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=1.2cm,
      minimum height=0.8cm,
      top color=yellow!10,
      bottom color=yellow!25,
      yellow batch stack
] (z1) at (\aonex, \noiserow) {\(z^1\)};

% Noise samples box with horizontal label
\node[draw,
      dashed,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1.5pt,
      fit=(zt) (z1),
      inner sep=0.6cm
] (noise_box) {};

% Add "Pre-generated noise" label (horizontal now)
\node[text=brown, font=\large, anchor=south] at ([yshift=0.3cm]noise_box.north) {\textbf{Pre-generated Gaussian Noise}};

% Define junction points between a0 and action nodes
\coordinate (junction1) at ($(a0.east)+(0.7,0)$);
\coordinate (junction2) at ($(junction1)+(0,-1.5)$);
\coordinate (upper_junction1) at ($(a0.east)+(0.7,0)$);
\coordinate (upper_junction2) at ($(upper_junction1)+(0,1.5)$);


\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=3cm,  % REDUCED width for more compact layout
      minimum height=0.5cm, 
      top color=orange!10,
      bottom color=orange!25,
      at={($(junction2)+(3.5cm,0)$)} % Adjusted position to center better
] (action) {};
% Create the sampling and noise nodes

% Create upper action node (normal sized)
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=2cm,
      minimum height=1.2cm,
      top color=orange!10,
      bottom color=orange!25,
      at={($(upper_junction2)+(3.5cm,0)$)},
      text width=1.8cm,
      align=center
] (upper_action) {\textbf{Discrete\\Actions}};

% Define midpoints for connections
\coordinate (lower_midpoint) at ($(junction2)!0.5!(action.west)$);
\coordinate (upper_midpoint) at ($(upper_junction2)!0.5!(upper_action.west)$);



% Create lower action node with vertical divisions (horizontal layout) - MADE MORE COMPACT

% Environment nodes - ADJUSTED POSITION
\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=2.5cm,
      minimum height=1cm,
      top color=purple!10,
      bottom color=purple!25,
      right=2cm of action.center,  % Closer to the action node
      label=center:{ \textbf{Continuous} \\ \textbf{Environment}}
] (env) {};

\node[draw,
      rounded corners=3pt,
      drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
      line width=1pt,
      minimum width=2.5cm,
      minimum height=1cm,
      top color=purple!10,
      bottom color=purple!25,
      right=2cm of upper_action.center,
      label=center:{ \textbf{Discrete} \\ \textbf{Environment}}
] (upper_env) {};

\coordinate (main_junction) at ($(S.north)+(0,0.8)$);

\coordinate (at_junction) at ($(main_junction -| at)$);
\coordinate (atm1_junction) at ($(main_junction -| atm1)$);
\coordinate (a2_junction) at ($(main_junction -| a2)$);
\coordinate (a1_junction) at ($(main_junction -| a1)$);
% \coordinate (a0_junction) at ($(main_junction -| a0)$);

% Draw the main stem from S to main_junction
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (S) -- (main_junction);

% Draw the horizontal junction line connecting all junction points
\draw[line width=1.2pt] (at_junction) -- (a1_junction);

% Draw vertical paths from junction to each a^t node
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (at_junction) -- (at);
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (atm1_junction) -- (atm1);
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (a2_junction) -- (a2);
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (a1_junction) -- (a1);

% Connect a0 to the action nodes through junctions (without the text labels)
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (a0) -- (junction1) -- (junction2) -- (action.west);
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (a0) -- (upper_junction1) -- (upper_junction2) -- (upper_action);

% Connect the new nodes to the midpoints

% Connect action nodes to environment nodes
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (action.east) -- (env) 
     node[midway, above, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {};
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (upper_action) -- (upper_env) 
     node[midway, above, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {};

% Vertical dividers for the horizontally flipped action node - ADJUSTED FOR COMPACT SIZE
\draw[line width=0.8pt] ($(action.north west)!0.25!(action.north east)$) -- ($(action.south west)!0.25!(action.south east)$);
\draw[line width=0.8pt] ($(action.north west)!0.5!(action.north east)$) -- ($(action.south west)!0.5!(action.south east)$);
\draw[line width=0.8pt] ($(action.north west)!0.75!(action.north east)$) -- ($(action.south west)!0.75!(action.south east)$);

% Action labels for the horizontal node compartments
\node at ($(action.west)!0.125!(action.east)$) {\textbf{a\(_1\)}};
\node at ($(action.west)!0.375!(action.east)$) {\textbf{a\(_2\)}};
\node at ($(action.west)!0.625!(action.east)$) {\textbf{a\(_3\)}};
\node at ($(action.west)!0.875!(action.east)$) {\textbf{a\(_4\)}};

% Action Sequence label (horizontal) - MOVED CLOSER
\node[below=0.1cm of action, text width=5cm, align=center] 
      {\textbf{Action Sequences}};

% Horizontal forward arrows
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (at) -- (atm1) 
     node[midway, above=0.5cm, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\scriptsize $\mu_\theta(a^t,t|S) +$ \\\scriptsize $\sigma_t z^t$};
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (atm1) -- (dots) 
     node[midway, above=0.5cm, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\scriptsize $\mu_\theta(a^{t-1},t|S) +$ \\ \scriptsize$\sigma_{t-1} z^{t-1}$};
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (dots) -- (a2) 
     node[midway, above=0.5cm, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\scriptsize $\mu_\theta(a^3,t|S) +$ \\ \scriptsize$\sigma_3 z^3$};
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (a2) -- (a1) 
     node[midway, above=0.5cm, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\scriptsize $\mu_\theta(a^2,t|S) +$ \\ \scriptsize$\sigma_2 z^2$};
\draw[-{Stealth[length=8pt]}, line width=1.2pt] (a1) -- (a0) 
     node[midway, above=0.5cm, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\scriptsize $\mu_\theta(a^1,t|S) +$ \\ \scriptsize$\sigma_1 z^1$};

% ----- NOISE INFLUENCE ARROWS (NOW VERTICAL) -----
\draw[-{Stealth[length=8pt]}, line width=1.2pt, color=blue!70, dashed] (zt) -- (at) 
     node[midway, right, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\(\sigma_t\)};
\draw[-{Stealth[length=8pt]}, line width=1.2pt, color=blue!70, dashed] (ztm1) -- (atm1) 
     node[midway, right, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\(\sigma_{t-1}\)};
\draw[-{Stealth[length=8pt]}, line width=1.2pt, color=blue!70, dashed] (z2) -- (a2) 
     node[midway, right, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\(\sigma_2\)};
\draw[-{Stealth[length=8pt]}, line width=1.2pt, color=blue!70, dashed] (z1) -- (a1) 
     node[midway, right, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {\(\sigma_1\)};

% Box 1: Forward denoising process
\node[draw=brown!70,
      dotted,
      line width=1.5pt,
      rounded corners=5pt,
      fill=brown,
      fill opacity=0.05,
      fit=(S) (at) (a0) (noise_box),
      inner sep=1cm,
      label={[text=brown!70, font=\bfseries\sffamily]above:{\textbf{Forward Denoising}}}
] (forward_box) {};

% Box 2: Environment interaction part
\node[draw=purple!70,
      dotted,
      line width=1.5pt,
      rounded corners=5pt,
      fill=purple,
      fill opacity=0.05,
      fit=(action) (env) (upper_action) (upper_env),
      inner sep=0.8cm,
      label={[text=purple!70, font=\bfseries\sffamily]above:Environment Interaction}
] (env_box) {};

% Add a subtle background
\begin{scope}[on background layer]
    \fill[gray!5, rounded corners=10pt] 
         ($(forward_box.north west)+(-0.5,0.5)$) rectangle 
         ($(env_box.south east)+(0.5,-0.5)$);
\end{scope}

% Add a title
% \node[font=\Large\bfseries\sffamily, text=black!80] 
%      at ($(forward_box.north)+(0,1.5)$) 
%      {Denoising Diffusion Policy};
     
\node[draw,
    rounded corners=3pt,
    drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
    line width=1pt,
    text width=2cm,
    align=center,
    font=\small\sffamily,
    top color=orange!10,
    bottom color=orange!25,
    above=0.8cm of upper_midpoint
] (sampling_logits) {Sampling\\from Logits};

\node[draw,
    rounded corners=3pt,
    drop shadow={shadow xshift=1pt, shadow yshift=-1pt, opacity=0.3},
    line width=1pt,
    text width=2cm,
    align=center,
    font=\small\sffamily,
    top color=yellow!10,
    bottom color=yellow!25,
    below=0.8cm of lower_midpoint
] (gaussian_noise) {Gaussian\\Noise};

\draw[-{Stealth[length=8pt]}, line width=1.2pt, color=blue!70] (gaussian_noise) -- (lower_midpoint)
     node[midway, right, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {};
\draw[-{Stealth[length=8pt]}, line width=1.2pt, color=blue!70] (sampling_logits) -- (upper_midpoint)
     node[midway, right, fill=white, fill opacity=0.7, text opacity=1, 
          rounded corners, inner sep=2pt] 
          {};
          
          
\end{tikzpicture}
}
    \caption{Denoising diffusion policy.}
    \label{fig:denoising_flow}
\end{figure}

==> sec/sec5-back.tex <==
\section{Experiments}

In this section, we provide a comprehensive evaluation of {\METHOD} across a variety of challenging environments. We begin by detailing the experimental setup in Sec.~\ref{sec:setup}, followed by results on continuous robot control tasks in Sec.~\ref{sec:continuous} and discrete multi-agent coordination tasks in Sec.\ref{sec:discrete}. Finally, we conduct ablation studies in Sec.~\ref{sec:ablation} to assess the robustness and of {\METHOD}.

For continuous robot control tasks, we compare \textbf{{\METHOD}} with standard Gaussian policies with MLP parametrization, \textbf{DPPO}~\citep{ren2024diffusion}; \textbf{DRWR} and \textbf{DAWR}~\citep{ren2024diffusion}, based on reward-weighted regression~\citep{peters2007reinforcement} and advantage-weighted regression respectively~\citep{peng2019advantage}; \textbf{DIPO}~\citep{yang2023policy}, which employs action gradients as the score function for denoising steps; and Q-learning-based methods such as \textbf{IDQL}~\citep{hansen2023idql} and \textbf{DQL} \citep{wang2022diffusion}. To further demonstrate the effectiveness of our PPO-based method over Q-function based methods, we also compare {\METHOD} against DAC~\citep{fang2024diffusion} and BDPO~\citep{gao2025behavior} in tasks with sparse rewards. To ensure a fair comparison, we adapted these methods in an offline-to-online manner by adding a replay buffer.

For the discrete multi-agent task Gooogle Research Football, we compare {\METHOD} with \yny{MLP policies trained using} Multi-Agent Proximal Policy Optimization (MAPPO) \citep{yu2022surprising}.
This baseline is initialized through behavior cloning using a Cross-Entropy loss function.


\subsection{Environmental Setup\label{sec:setup}}

\textbf{Environments: OpenAI Gym locomotion.} Our first set of experiments involves testing {\METHOD} on a series of well-established locomotion benchmarks from OpenAI Gym \citep{brockman2016openai}, namely: \texttt{Hopper-v2}, \texttt{Walker2D-v2}, and \texttt{HalfCheetah-v2}. The pre-trained Diffusion Policies used in these experiments are trained from the D4RL "medium" dataset \citep{fu2020d4rl}, which contains a diverse range of pre-recorded trajectories. For the fine-tuning process, we use \textbf{dense} reward. 

\textbf{Environments: Franka Kitchen.} We also evaluate the performance of {\METHOD} on Franka Kitchen benchmarks~\citep{gupta2019relay}. In this environment, agents need to complete four sub-tasks with a certain order. The datasets for pretraining are \texttt{complete}, \texttt{mixed} and \texttt{partial} in D4RL dataset~\citep{fu2020d4rl}. All tasks are fine-tuned using \textbf{sparse} rewards, which gives reward of 1 when one sub-task is completed.

\textbf{Environments: Robomimic.} We further evaluate the performance of {\METHOD} on robotic manipulation tasks within Robomimic benchmarks~\citep{robomimic2021}. The specific scenarios we consider include \texttt{Lift}, \texttt{Can}, \texttt{Square}, and \texttt{Transport}, varying in difficulty. To ensure temporal consistency in actions, we employ action chunking with size 4 for \texttt{Lift}, \texttt{Can}, and \texttt{Square}, and size 8 for \texttt{Transport}, following the setting in~\citep{ren2024diffusion}. All tasks are fine-tuned using \textbf{sparse} rewards, which provide feedback only in the form of success or failure signals. 

\textbf{Environments: Google Research Football.} 
To evaluate {\METHOD}'s capability in large discrete action spaces, we test on three Google Research Football scenarios requiring multi-agent coordination: \texttt{3 vs 1 with Keeper}, \texttt{Counterattack Hard}, and \texttt{Corner}.
 \yny{Here we adopt a centralized control strategy, where actions for all agents are generated simultaneously using a single Diffusion Policy. The base Diffusion Policies are pre-trained to output one-hot vectors corresponding to ground-truth actions. To construct the pre-training dataset, we aggregate trajectories from multiple MLP-based policies with varying success rates.} 
 
 As no public dataset exists for Google Research Football, a custom dataset \yny{is} constructed to pre-train Diffusion Policies by training multiple MAPPO agents~\citep{yu2022surprising} with different random seeds and early-stopping them at various stages. These agents exhibit varying winning rates and employ diverse tactical behaviors.



\subsection{Evaluation on Continuous Robot Control Tasks}\label{sec:continuous}
From the experimental results shown in Fig.~\ref{fig:merged} and Table.~\ref{table:performance_auto}, we observe that {\METHOD} consistently achieves the strongest performance, exhibits robustness and the highest sample efficiency across all tasks. 


\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/merged.png}
    \caption{Performance comparison on OpenAI Gym locomotion, Franka Kitchen and Robomimic tasks. Results are averaged over three seeds. {\METHOD} (ours) achieves the strongest performance.}
    \label{fig:merged}
\end{figure}

These experimental results also suggest methods that rely on Q-funtion estimation generally underperform in complex tasks with long horizons and sparse reward signals, like the Franka Kitchen and Robomimic tasks. This may be due to increased difficulty in obtaining an accurate Q-function in such scenarios.


We also conducted experiments with \textbf{visual inputs} on the toughest two tasks \texttt{Square} and \texttt{Transport} in Robomimic environment in Fig.~\ref{fig:robomimic-vision}. To our surprise, our method {\METHOD} achieves remarkable \textbf{performance improvement} and \textbf{much higher sample-efficiency} (about 4 times faster than DPPO) in these hardest visual tasks. These results highlight our superioirity in real-world applications. These results confirms the effectiveness of our methods in tasks close to real-world applications.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/robomimic-vision.png}
    \caption{Performance comparison on Robomimic visual tasks. Results are averaged over three seeds. {\METHOD} (ours) achieves the strongest performance. VIT-MLP uses Vision Transformer for encoding image observations and generates a Gaussian policy.}
    \label{fig:robomimic-vision}
\end{figure}


\subsection{Evaluation on Discrete Multi-agent Coordination Tasks}\label{sec:discrete}
Following our evaluation on continuous control tasks, we next examine {\METHOD} on Google Research Football, a benchmark for cooperative multi-agent control. 






\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/football.png}
    \caption{Performance comparison in Google Research Football. Results are averaged over at least three seeds. {\METHOD} (ours) exhibits strong performance and stability.}
    \label{fig:football}
\end{figure}

% \yny{To facilitate more effective coordination among agents, we adopt a centralized multi-agent control strategy in which actions for all agents are generated simultaneously. This formulation leverages the high representational capacity of diffusion models to model complex inter-agent dependencies. However, it also gives rise to a high-dimensional joint action space (i.e., $\text{num\_agents} \times \text{actions}$), presenting substantial challenges for reinforcement learning fine-tuning.}
As Fig.~\ref{fig:football} and Table.~\ref{table:football} demonstrates, {\METHOD} outperforms the MLP baseline across all three evaluated scenarios. This outcome not only highlights the superiority of Diffusion Policy in handling complex and diverse demonstration data over simple MLP policy, but also confirms the effectiveness of the DP+{\METHOD} during the fine-tuning phase.






\subsection{{\METHOD} is Robust to the Number of Denoising Steps\label{sec:ablation}}


We further conduct studies to investigate the impact of varying the number of denoising steps in the diffusion model. The experimental results shown in Fig.~\ref{fig:ablation-denoise_step} indicate that {\METHOD} demonstrates strong robustness to the choice of denoising steps.




\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/gym-denoise.png}
    \caption{Ablation Study on Denoising Steps in OpenAI Gym locomotion tasks.}
    \label{fig:ablation-denoise_step}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/robomimic-denoising-step.png}
    \caption{Ablation Study on Denoising Steps in Robomimic tasks.}
    \label{fig:ablation-denoise_step}
\end{figure}


We hypothesize that the robustness of {\METHOD} arises from the way gradients are propagated through time during the diffusion process. This gradient flow leads to more accurate gradient estimates.

